DIVKNOWQA: Assessing the Reasoning Ability of LLMs via Open-Domain Question Answering over Knowledge Base and Text

Large Language Models (LLMs) have exhibited impressive generation capabilities, but they suffer from hallucinations when solely relying on their internal knowledge, especially when answering questions that require less commonly known information. Retrieval-augmented LLMs have emerged as a potential solution to ground LLMs in external knowledge. Nonetheless, recent approaches have primarily emphasized retrieval from unstructured text corpora, owing to its seamless integration into prompts. When using structured data such as knowledge graphs, most methods simplify it into natural text, neglecting the underlying structures. Moreover, a significant gap in the current landscape is the absence of a realistic benchmark for evaluating the effectiveness of grounding LLMs on heterogeneous knowledge sources (e.g., knowledge base and text). To fill this gap, we have curated a comprehensive dataset that poses two unique challenges: (1) Two-hop multi-source questions that require retrieving information from both open-domain structured and unstructured knowledge sources; retrieving information from structured knowledge sources is a critical component in correctly answering the questions. (2) The generation of symbolic queries (e.g., SPARQL for Wikidata) is a key requirement, which adds another layer of challenge. Our dataset is created using a combination of automatic generation through predefined reasoning chains and human annotation. We also introduce a novel approach that leverages multiple retrieval tools, including text passage retrieval and symbolic language-assisted retrieval. Our model outperforms previous approaches by a significant margin, demonstrating its effectiveness in addressing the above-mentioned reasoning challenges.

==> examples/718_example.tex <==
target Q: How many awards has the first person to walk on the moon received?
target A: ['26', 'twenty-six']

pred A:26

retrieve_answer A:26
sparql_answer A:26

EM:True

HotPotF1:1.0

Recall:True



**********hop_0**********

Write a search query, query entity, and sparql that will help answer a complex question.

---

Follow the following format.

Context:
${sources that may contain relevant content}

Question: ${the question to be answered}

Rationale: Let's think step by step. Based on the context, we have learned the following. ${information from the context that provides useful clues}

Search Query: ${a simple question for seeking the missing information}

Query Entity: ${query entity name from search query}

---

Context:


Question: what are the occupations of the person who holds the most women's wimbledon titles?

Rationale: Let's think step by step. Based on the context, we have learned the following. Decompose the question to answer the following single hop questions. 1. who holds the most women's wimbledon titles? 2. what are the occupations of this person

Search Query: who holds the most women's wimbledon titles?

---

Context:


Question: Which bay is the name of David Resnick's place of birth?

Rationale: Let's think step by step. Based on the context, we have learned the following. Decompose the question to answer the following single hop questions. 1. where was David Resnick born? 2. which bay is the name of this place

Search Query: where was David Resnick born?

Query Entity: David Resnick

---

Context:


Question: Is the person who direct the film the shape of water a member of Writers Guild of America, West?

Rationale: Let's think step by step. Based on the context, we have learned the following. Decompose the question to answer the following single hop questions. 1. who direct the film the shape of water? 2. Is the person the person a member of Writers Guild of America, West?

Search Query: director of the film the shape of water

---

Context:


Question: How many awards has the first person to walk on the moon received?

Rationale: Let's think step by step. Based on the context, we have learned the following.
Rationale: Decompose the question to answer the following single hop questions. 1. who is the first person to walk on the moon? 2. how many awards has this person received?
Query: first person to walk on the moon

Rationale: Decompose the question to answer the following single hop questions. 1. who was the first person to walk on the moon? 2. how many awards has this person received?
Query: first person to walk on the moon

Rationale: Decompose the question to answer the following single hop questions. 1. who was the first person to walk on the moon? 2. how many awards has this person received?
Query: first person to walk on the moon
Entity Name : None
Entity ID : None
Relation Name : None
Relation ID : None
SPARQL : None
Answer : None

**********hop_1**********

Write a search query, query entity, and sparql that will help answer a complex question.

---

Follow the following format.

Context:
${sources that may contain relevant content}

Question: ${the question to be answered}

Rationale: Let's think step by step. Based on the context, we have learned the following. ${information from the context that provides useful clues}

Search Query: ${a simple question for seeking the missing information}

Query Entity: ${query entity name from search query}

---

Context:
[1] «The Wimbledon Championships, commonly known simply as Wimbledon,[c] is the oldest tennis tournament in the world and is widely regarded as the most prestigious.[2][3][4][5][6] It has been held at the All England Club in Wimbledon, London, since 1877 and is played on outdoor grass courts, with retractable roofs over the two main courts since 2019.»
[2] «These records only include the Open Era, since the inclusion of the professional tennis players, Martina Navratilova (1978–1979, 1982–1987, 1990) holds the record for most victories with nine.»

Question: what are the occupations of the person who holds the most women's wimbledon titles?

Rationale: Let's think step by step. Based on the context, we have learned the following. Wimbledon is tennis tournament, and tennis player Martina Navratilova holds the most women's wimbledon titles. The second step is to answer what are the occupations of this person?

Search Query: what are the occupations of Martina Navratilova?

---

Context:
«where was David Resnick born? Rio de Janeiro»

Question: Which bay is the name of David Resnick's place of birth?

Rationale: Let's think step by step. Based on the context, we have learned the following. David Resnick is born in Rio de Janeiro. The second step is to answer which bay is the name of Rio de Janeiro?

Search Query: which bay is the name of Rio de Janeiro?

Query Entity: David Resnick

---

Context:
«The Shape of Water is a 2017 American romantic dark fantasy drama film directed by Guillermo del Toro and written by del Toro and Vanessa Taylor.[3][4] It stars Sally Hawkins, Michael Shannon, Richard Jenkins, Doug Jones, Michael Stuhlbarg, and Octavia Spencer. Set in Baltimore in 1962, the story follows a mute custodian at a high-security government laboratory who falls in love with a captured humanoid amphibian creature.»

Question: Is the person who direct the film the shape of water a member of Writers Guild of America, West?

Rationale: Let's think step by step. Based on the context, we have learned the following. The Shape of Water is directed by Guillermo del Toro. The second step is to answer is the person a member of Writers Guild of America, West

Search Query: the organization Guillermo del Toro is in

---

Context:
[1] «. Neil Armstrong v17 type : influence influence node . Neil Armstrong v17 type : book book subject . Neil Armstrong v17 description : Neil Alden Armstrong was an American astronaut and the first person to walk on the Moon  He was also an aerospace engineer, naval aviator, test pilot, and university professor  Before becoming an astronaut, Armstrong was an officer in the U S  Navy and served in the Korean War  After the war, he earned his bachelor's degree at Purdue University and served as a test pilot at the National Advisory Committee for Aeronautics»
[2] «place of birth San Francisco v83 . John Young v13 spaceflight astronaut missions Apollo 16 . John Young v13 spaceflight astronaut space time minutes 50139.0 . John Young v13 description : Captain John Watts Young is a retired American astronaut, naval officer and aviator, test pilot, and aeronautical engineer, who became the ninth person to walk on the Moon as Commander of the Apollo 16 mission in 1972 \nYoung enjoyed the longest career of any astronaut, becoming the first person to make six space flights over the course of 42 years of active NASA service, and is the only person»
[3] «fourth human lunar landing  He was the eighth person to walk on the Moon and the first, and youngest, of those astronauts to die  . James Irwin type : base type ontology animate . James Irwin type : common topic . James Irwin type : spaceflight astronaut . James Irwin type : base type ontology agent . James Irwin type : people person . James Irwin prominent type : spaceflight astronaut .»
[4] «She was the first female newscaster on television in Los Angeles and the West Coast  She has received many awards and honors, including a Lifetime Achievement Emmy Award and a star on the Hollywood Walk of Fame  . Ruth Ashton Taylor prominent type : people person . Ruth Ashton Taylor type : base type ontology animate . Ruth Ashton Taylor type : common topic . Ruth Ashton Taylor type : base type ontology agent . Ruth Ashton Taylor type : people person .»
[5] «Congressional Gold Medal, the highest civilian award in the United States. The bill was sponsored by Florida Senator Bill Nelson and Florida Representative Alan Grayson. A group of British scientists interviewed as part of the anniversary events reflected on the significance of the Moon landing: Apollo 11 Apollo 11 was the spaceflight that landed the first two people on the Moon. Commander Neil Armstrong and Lunar Module Pilot Buzz Aldrin, both American, landed the lunar module "Eagle" on July 20, 1969, at 20:17 UTC. Armstrong became the first person to step onto the lunar surface six hours after landing»

Question: How many awards has the first person to walk on the moon received?

Rationale: Let's think step by step. Based on the context, we have learned the following.
Rationale: Neil Armstrong was the first person to walk on the moon. The second step is to answer how many awards he has received.
Query: how many awards has Neil Armstrong received?

Rationale: Neil Armstrong was the first person to walk on the moon. The second step is to answer how many awards he has received.
Query: how many awards has Neil Armstrong received?

Rationale: The first person to walk on the moon is Neil Armstrong. The second step is to answer how many awards he has received.
Query: how many awards has Neil Armstrong received?
Entity Name : Neil Armstrong
Entity ID : Q1615
Relation Name : award received
Relation ID : P166
SPARQL : SELECT (COUNT(?award) as ?count) WHERE { wd:Q1615 wdt:P166 ?award. }
Answer : 26

**********QA_Step**********

Answer questions with short factoid answers.

---

Follow the following format.

Context:
${sources that may contain relevant content}

Question: ${the question to be answered}

Rationale: Let's think step by step. ${a step-by-step deduction that identifies the correct response, which will be provided below}

Answer: ${a short factoid answer, often between 1 and 5 words}

---

Context:
[1] «Martina Navratilova (Czech: Martina Navrátilová [ˈmarcɪna ˈnavraːcɪlovaː] (listen); née Šubertová [ˈʃubɛrtovaː]; born October 18, 1956) is a Czech–born American former professional tennis player. Widely considered among the greatest tennis players of all time, Navratilova won 18 major singles titles, 31 major women's doubles titles, and 10 major mixed doubles titles, for a combined total of 59 major titles, the most in the Open Era.[3][4] Alongside Chris Evert, her greatest rival, Navratilova dominated women's tennis in the 1970s and 1980s.»
[2] «Martina Navratilova occupation writer .  Martina Navratilova occupation novelist . Martina Navratilova occupation tennis player . Martina Navratilova occupation autobiographer .»

Question: what are the occupations of the person who holds the most women's wimbledon titles?

Rationale: Let's think step by step. Martina Navratilova is a tennis player, writer, novelist, and autobiographer.

Answer: tennis player, writer, novelist, and autobiographer

---

Context:
«"Rio de Janeiro" was the name of Guanabara Bay»

Question: Which bay is the name of David Resnick's place of birth?

Rationale: Let's think step by step. David Resnick was born in Rio de Janeiro, and "Rio de Janeiro" was the name of Guanabara Bay.

Answer: Guanabara Bay

---

Context:
[1] «Guillermo del Toro Gómez (Spanish: [ɡiˈʝeɾmo ðel ˈtoɾo]; born 9 October 1964) is a Mexican filmmaker and author. A recipient of three Academy Awards, three BAFTA Awards, and an Emmy Award, his work has been characterized by a strong connection to fairy tales and horror, with an effort to infuse visual or poetic beauty in the grotesque.[4] He has had a lifelong fascination with monsters, which he considers symbols of great power.[5] He is also known for his use of insectile and religious imagery, his themes of Catholicism, anti-fascism, and celebrating imperfection, underworld motifs, practical special effects, dominant amber lighting, and his frequent collaborations with actors Ron Perlman and Doug Jones.[6][7]»
[2] «Guillermo del Toro Gómez member of Writers Guild of America, West . »

Question: Is the person who direct the film the shape of water a member of Writers Guild of America, West?

Rationale: Let's think step by step. Guillermo del Toro Gómez is a filmmaker, he is a member of Writers Guild of America, West .

Answer: yes

---

Context:
[1] «Neil Armstrong was the first person to walk on the moon. The second step is to answer how many awards he has received.»
[2] «how many awards has Neil Armstrong received?	26»
[3] «award received Langley Gold Medal . Neil Armstrong award received Silver Buffalo Award . Neil Armstrong award received Livingstone Medal . Neil Armstrong award received star on Hollywood Walk of Fame . Neil Armstrong award received Grande Médaille d'Or des Explorations . Neil Armstrong award received International Space Hall of Fame . Neil Armstrong ISNI 0000 0001 2147 959X . Neil Armstrong military branch United States Navy . Neil Armstrong part of NASA Astronaut Group 2 . Neil Armstrong military rank lieutenant (junior grade) . Neil Armstrong astronaut mission Apollo 11 . Neil Armstrong astronaut mission Gemini 8 . Neil»
[4] «award received Order of the Yugoslav Star . Neil Armstrong award received Air Medal . Neil Armstrong award received Collier Trophy . Neil Armstrong award received Congressional Space Medal of Honor . Neil Armstrong award received National Defense Service Medal . Neil Armstrong award received Korean Service Medal . Neil Armstrong award received Eagle Scout . Neil Armstrong award received NASA Distinguished Service Medal . Neil Armstrong award received Hubbard Medal . Neil Armstrong award received Sylvanus Thayer Award . Neil Armstrong award received Arthur S. Flemming Award . Neil Armstrong award received Distinguished Eagle Scout Award . Neil Armstrong»
[5] «Armstrong employer University of Cincinnati . Neil Armstrong signature http://commons.wikimedia.org/wiki/Special:FilePath/Neil%20Armstrong%20Signature.svg . Neil Armstrong place of burial Atlantic Ocean . Neil Armstrong religion or worldview deism . Neil Armstrong award received Presidential Medal of Freedom . Neil Armstrong award received Order of the White Elephant . Neil Armstrong award received Cullum Geographical Medal . Neil Armstrong award received National Aviation Hall of Fame . Neil Armstrong award received Order of Culture . Neil Armstrong award received United Nations Medal . Neil Armstrong award received Congressional Gold Medal . Neil Armstrong award received United States Astronaut Hall of Fame . Neil Armstrong»
[6] «She was the first female newscaster on television in Los Angeles and the West Coast  She has received many awards and honors, including a Lifetime Achievement Emmy Award and a star on the Hollywood Walk of Fame  . Ruth Ashton Taylor prominent type : people person . Ruth Ashton Taylor type : base type ontology animate . Ruth Ashton Taylor type : common topic . Ruth Ashton Taylor type : base type ontology agent . Ruth Ashton Taylor type : people person .»
[7] «Congressional Gold Medal, the highest civilian award in the United States. The bill was sponsored by Florida Senator Bill Nelson and Florida Representative Alan Grayson. A group of British scientists interviewed as part of the anniversary events reflected on the significance of the Moon landing: Apollo 11 Apollo 11 was the spaceflight that landed the first two people on the Moon. Commander Neil Armstrong and Lunar Module»

Question: How many awards has the first person to walk on the moon received?

Rationale: Let's think step by step.

majority completions 

Rationale: Neil Armstrong was the first person to walk on the moon and he has received 26 awards.

Answer: 26



==> tables/dataset_comparision_v2.tex <==
\begin{table}[!t]
\centering
\small
\caption{\label{tab:dataset-property}
Comparing benchmarks for heterogeneous QA. OpenR: Open Retrieval; Human: Human Questions; EI: Equitable Importance Knowledge Source; SG: Structured Ground-truth.
}

\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|ccc|cccc}
\toprule
\textbf{Dataset} & \textbf{Heterogenous} & \textbf{OpenR} & \textbf{Human}& \textbf{EI} & \textbf{SG} \\
\hline
HybridQA~\citep{chen2021ottqa} & \xmark & \cmark &  \cmark & \xmark & \cmark & \cmark & \xmark
\\ 
OTT-QA~\citep{chen2020hybridqa} & \xmark & \cmark &  \cmark & \cmark & \cmark & \cmark & \xmark
\\ 
NQ-Tables~\citep{herzig2021open} & \xmark & \cmark &  \cmark & \xmark & \xmark & \xmark & \xmark
\\ 
TAT-QA ~\citep{zhu2021tat} & \xmark & \cmark &  \cmark & \xmark & \cmark & \cmark & \xmark
\\ 
MultimodelQA~\citep{talmor2021multimodalqa} & \xmark & \cmark &  \cmark & \xmark & \cmark & \xmark & \xmark
\\ 
Manymodelqa ~\citep{hannan2020manymodalqa} & \xmark & \cmark &  \cmark & \xmark & \cmark & \xmark & \xmark
\\ 
FinQA ~\citep{chen-etal-2021-finqa} & \xmark & \cmark &  \cmark & \xmark & \cmark & \cmark & \xmark
\\ 
HetpQA ~\citep{shen-etal-2022-product} & \xmark & \cmark &  \cmark & \xmark & \cmark & \xmark & \xmark
\\ 
CompMix ~\citep{christmann2023compmix} & \xmark & \cmark &  \cmark & \cmark & \cmark & \xmark & \xmark
\\
WikiMovies-10K ~\citep{miller2016key} & \cmark & \cmark &  \xmark & \cmark & \cmark & \xmark & \xmark \\
MetaQA ~\citep{zhang2018variational} & \cmark & \cmark &  \xmark & \cmark & \cmark & \xmark & \xmark \\

\midrule
\dataset (Ours) & \cmark & \cmark &  \xmark & \cmark & \cmark & \cmark & \cmark 
\\
\bottomrule
\end{tabular}
}
\vspace{-1em}
\end{table}

==> tables/main_table_oct12_breakdown.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]

\centering
\caption{Breakdown Analysis of Answer and Sub-Step Retrieval Accuracy on \dataset.}
\label{table:main-table-breakdown} 
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lllllll}
\hline
                         &     Knowledge              & 1/short & 1/agg & 1/y & 2/short & 2/y\\
\hline
\multirow{3}{*}{ChatGPT} & None        &   27.2  &  27.3 & \textbf{33.3}  & \textbf{33.3}  &  27.7 \\
                        & Text(bm25)    &  21.5  & 20.7  & 28.6  & 28.2 & 27.7  \\
                     & Text(Contriever)    &   14.7  & 20.2  &  21.4 &  27.2 &  23.4 \\
                     & KB     &  17.8  & 22.7  & 28.0  & 28.2  &  21.8 \\
                      % & Text + KB *    &  19.9  & 22.7  &  24.4 & 29.2   & 26.6   \\
                    & Text + KB *    &  19.9  & 23.2  &  25.0 & 29.7   & 26.6   \\
% \hline
% CoT  & None       &  20.9  &  21.7 & 18.5  &  20.5 & 18.6  \\


% \hline

% \multirow{2}{*}{ReAct}      & Text             &     &    &   &   & \\
%                             & KB             &     &    &   &   & \\
% ReAct     & Wikipedia              &    &   &   &   &   \\
\hline
\multirow{3}{*}{DSP}      & Text(BM25)      & 18.8   & 19.2  & 14.9  &  18.5 &  22.3 \\
& Text(contriever)     &  17.3  & 19.2  & 21.4  & 23.6  &  20.7 \\
                            & KB       &  22.0  & 21.7  & 19.0  &26.7& 25.0  \\

\hline
\multirow{3}{*}{\approach}    & Text(BM25) + KB     & 23.0   &  25.3 & 23.2  & 27.7  &  23.4 \\
 & \textbf{Text(BM25) + KB + SPARQL}   & 27.7   & 29.8  & 28.0  &  32.8 & 26.6  \\
 
& Text(Contriever) + KB    &  28.8  &  26.8 &  23.8 & 31.8  &  28.7 \\

 & \textbf{Text(Contriever) + KB + SPARQL}   & \textbf{36.1}   & \textbf{30.3}  & 20.8  & \textbf{32.3}  &  \textbf{31.4} \\
 
\hline
\end{tabular}
\vspace{-1em}
}
\end{table*}








==> tables/main_table_oct17.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\centering
\caption{
\label{table:main-table} 
Answer and Sub-Step Retrieval Accuracy on \dataset on Tool-Augmented LLMs.}
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{lllllll}
\hline
                         &     Knowledge              & EM & F1 & Recall & H1-R &  H2-R \\
\hline
\multirow{4}{*}{Vanilla Prompt} & None     & 30.2  & 33.8  & 31.2   & - \\
 & Text(bm25)     & 25.1  &27.7  &   26.1 &  42.9  &  -  \\
  & Text(Contriever)     & 25.7  & 28.1 & 26.7  & 48.1  & - \\
 & KB     & 25.5  & 27.3 & 26.9  & 43.6  & -   \\
 % & Text + KB*    &  25.9  & 28.2  &  26.7 & -   & -   \\
  & Text + KB*    &  26.0 &  28.3  & 26.8 &   42.2  & -   \\
\hline
% CoT  & None     & 20.7  & 23.8 & 24.0  &  - & -   \\
% \hline

% \multirow{3}{*}{ReAct}      & Text    &   5.85 & 6.31 & 1.06  & -  & -    \\
% & KB              &  8.94 &  9.87  &  17.0 & - & -    \\
% & Text + KB*         & 8.19  & 9.76 &  2.13 &  - & -    \\
ReAct & Text + KB*         & 7.66 & 8.97 & 8.94  &  - & -    \\
\hline
\multirow{4}{*}{DSP}      & Text(BM25)     & 21.5  & 24.3 & 24.7  & 45.0  &   30.4  \\

& Text(contriever)   &  22.4 & 26.2 & 26.8  & 57.0   & 34.5\\
& KB      & 24.1  & 26.6 & 27.9  &46.3   &   31.0 \\
% & Text[oracle]    & 26.5   & 31.4  & 32.8  &  96.4  & 51.8  \\
& Text+KB*    & 27.9   & 31.0  & 31.2  &  57.6  & 41.2  \\

\hline
\multirow{3}{*}{\approach}    & Text(BM25) + KB    & 26.4  & 29.8 &30.2   & 60.0  &   41.2 \\
 &Text(BM25) + KB + SPARQL  & 28.5   & 31.8  & 32.0  & 61.5  &   42.1  \\
 
& Text(Contriever) + KB    & 30.7  & 35.0 &  35.5 & 68.9  &  46.8  \\

 & \textbf{Text(Contriever) + KB + SPARQL} & \textbf{32.1}  & \textbf{35.7} & \textbf{35.6}  &\textbf{70.1}   &  \textbf{47.1}  \\
\hline
\end{tabular}
\vspace{-1em}
}
\end{table*}








==> tables/question_example.tex <==
\begin{table*}[!t]
% \renewcommand{\arraystretch}{1.3}
\centering
\caption{\label{tab:dataset-type}
Types of multi-hop reasoning required to answer questions in \dataset. \shafiq{can you fix the last box's vertical line}. \shafiq{Show which questions are coming from NQ and which one is constructed from KB (show triplet for that).}
}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\textbf{Order} &  \textbf{Type} &\textbf{\%} & \textbf{Example} \\
\midrule

 & short entity & 20.3  &  \makecell{Q1: Who is Rafael Nadal married to?\\
Q1-A: María Francisca Perelló\\
Triplet: (Rafael Nadal, spouse, María Francisca Perelló)\\
Q2: Who won the Men's US Open 2017?\\
Q2-A: Rafael Nadal\\
Question: Who is the person married to the winner of the Men's US Open 2017?\\
Answer: María Francisca Perelló}
\\ 
\cline{2-4}
{Text $\rightarrow$ KB}  & yes/no &  17.9 &  \makecell{Q1: Who sang When the Lights Went Out in Georgia?\\
Q1-A: Vicki Lawrence\\
Triplet: (Vicki Lawrence, hair color, red hair)\\
Q2: What is Vicki Lawrence's hair color?\\
Q2-A: red hair\\
Question:  Is the hair color of the singer of "When the Lights Went Out in Georgia" gray?\\
Answer: no}
\\ 
\cline{2-4}
  & aggregate & 21.1  &  \makecell{Q1: who does Meg 's voice on Family Guy?\\
Q1-A: Vicki Lawrence\\
Triplet: (Mila Kunis, child, [Wyatt Kutcher, Dimitri Kutcher])\\
Q2: How many children does Mila Kunis have?\\
Q2-A: Two\\
Question: How many children does the person who does Meg's voice on Family Guy have?\\
Answer: Two} 
\\ 
\midrule
% \multirow{2}{*}{KB $\rightarrow$ Text}
% \makecell{ Q\\ Q\\ Q\\ KB $\rightarrow$ Text Q\\ Q\\ Q\\}
% \multirow{8}{*}{ \begin{tabular}{l}
%     {KB $\rightarrow$ Text}
% \end{tabular} }
\multirow{8}{*}{ 
    {KB $\rightarrow$ Text}
 }
& short entity & 20.7  &  
\makecell{Triplet: (William Weatherall Wilkins, present in work, Mary Poppins Returns)\\
Q1: In which work is William Weatherall Wilkins present?\\
Q1-A: Mary Poppins Returns\\
Q2: Who play Mary Poppins in Mary Poppins Returns?\\
Q2-A: Emily Blunt\\
Question: Who plays Mary Poppins in the work in which William Weatherall Wilkins is present?\\
Answer: Emily Blunt} \\
% {KB $\rightarrow$ Text} 
\cline{2-4}
& yes/no &  20.0 &  \makecell{Triplet: (Girl \#2, present in work, High School Musical) \\
Q1: In which work is Girl \#2 present?\\
Q1-A: High School Musical\\
Q2: What grade were they in in high school musical 1?\\
Q2-A: juniors\\
Question: Were they seniors in the work in which Girl \#2 is present?\\
Answer: no}
\\ 
\bottomrule
\end{tabular}
}
\vspace{-1em}
\end{table*}


==> tables/table_1_breakdown.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
        Prompt Step                 &      Available Resource              & EM & F1 & Recall & Retrieval Acc & hop1-acc\\
\hline
\multirow{3}{*}{Single} & w/o retrieval       &  0   &   9 &  0 &   - &  \\
                             & Text               &  1.2   & 8.3   & 1.2  & 7.9 &  \\
                             & KB               &   0.4  & 5.3   & 0.8  &  2.4 &  \\
\hline
\multirow{3}{*}{Multi}  & w/o retrieval      &  0.8   &  11.7  & 1.2  & -   & \\
                             & KB                 &   0.4  & 7.0     & 0.4  & 2.7  & 8.70 \\

\hline
\multirow{3}{*}{Sparse}       & Text               &   0.8    & 9.8  & 0.8  &7.9  &  11.86 \\
                             & Text + KB          &  0.8    &  9.1  & 1.2  & 7.9  & 13.04  \\
                             & Text + KB (SAPRQL) &   1.2    & 10.5    & 1.6  & 8.7  &  30.83 \\
\hline
\multirow{3}{*}{Dense}      & Text               &    2.4   & 11.0  & 3.6  &  13.8 &  17.00  \\
                             & Text + KB          &  2.8     & 11.7   &  4.3 &  13.43 &  13.83  \\
                             & Text + KB (SAPRQL) &   5.1   & 16.5    & 6.3 &  16.2 &  28.85  \\
\hline
\end{tabular}
\caption{Experiment results w.r.t final answer}
\end{table}








==> tables/table_1_kbtext_main.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\centering
\caption{Experiment results on KB\&Text short entity type questions.}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
        Prompt Step                 &      Available Resource              & EM & F1 & Recall & Retrieval Acc & hop1-acc\\
\hline
\multirow{3}{*}{Single} & w/o retrieval       &   20.5   &  27.3  & 26.5  &   - & - \\
                             & Text             & 14.0    &  18.1  &  15.8 &  25.5   & - \\
                             & KB             &  7.2   &  11.8  &  10.2 & 12   & - \\
\hline
CoT  & w/o retrieval       &  16.2   &  23.0  & 22.0  &  -  & - \\


\hline
\multirow{5}{*}{Dense}      & Text             &  16   & 21.6   &  20.0 &   14.3 & 31   \\
                            & KB             &  17.2   & 24.2  &  21.0 & 21.5 & 52.5    \\

                              & \textbf{Text + KB}        &   24.9  & 33.1   & 31.8  &  40.68  &  46.42 \\
                             & \textbf{Text + KB (SAPRQL)}   &  \textbf{25.2}  &  32.9  &  31.4   &  \textbf{43.61}    &  \textbf{52.99} \\
\hline
\end{tabular}
\vspace{-1em}
\end{table}







